Robotic Barrier Construction through Weaved, Inflatable Tubes

In this article, we present a mechanism and related path planning algorithm to construct light-duty barriers out of extruded, inflated tubes weaved around existing environmental features. Our extruded tubes are based on everted vine-robots and in this context, we present a new method to steer their growth. We characterize the mechanism in terms of accuracy resilience, and, towards their use as barriers, the ability of the tubes to withstand distributed loads. We further explore an algorithm which, given a feature map and the size and direction of the external load, can determine where and how to extrude the barrier. Finally, we showcase the potential of this method in an autonomously extruded two-layer wall weaved around three pipes. While preliminary, our work indicates that this method has the potential for barrier construction in cluttered environments, e.g. shelters against wind or snow. Future work may show how to achieve tighter weaves, how to leverage weave friction for improved strength, how to assess barrier performance for feedback control, and how to operate the extrusion mechanism off of a mobile robot.

==> KP_notes.tex <==


To Do:
- Give Haron feedback
- Add bulletpointed list with contents under each section
- Get details on hardware
- Write intro
- Write related work
-- Vine robots
-- Other methods for reconfiguration
-- Environmental barriers
-- Collective Robotic Construction?
-- Found materials (rock stacking)
-- https://journals-sagepub-com.proxy.library.cornell.edu/doi/full/10.1177/0278364915587925?casa_token=ILRH0rDKCOoAAAAA%3AtlGz7bf-ylR7CWkWINouii1_lqWdVGaakg2a_lFlYAIkNcy99cAxbg4tU0-1jKxE5-k5DXfnEB-T

%%%%%%%%%%%%%%%%%%%%%%%%%%

Intro:










%%%%%%%%%%%%%%%%%%%%%%%%%%

- Benefits to construction with inflated, weaved structures:
-- Minimal building material, less waste, bigger structures per load
-- Weaving brings added strength?
-- It allows us to use existing features in the landscape as anchor points to strengthen structures
-- Our reconfiguration version makes planning easier?

- Places where this could be useful
-- Wind/rain/snow shelters
-- Sun shelters
-- How to create shelter from the wind
-- Avalanche protection
-- Rain shelters
-- Soil stabilization??
-- Containment fences
-- Protecting fragile ecosystems

Current materials:
-- Tarps 
-- flexible low density polyethylene

- Issues:
-- These inflated beam robots tend to buckle under compressive loads, producing extremely tight local curvature at difficult-to-control buckle point locations.

- Directional steering
Methods of actuating everting vine robot growth direction and shape, including (top) actuation principles and (bottom) examples of implementation. (A) Distributed strain uses pneumatic artificial muscles to create strain along the length where they are attached. (B) Concentrated strain uses tendons actuated from the base to change the robot shape. (C) Tip-localized strain couples steering and growth to create responsive steering at the tip only. (D) Preformed steering shapes the robot for known tasks before deployment.
(A example) Series pneumatic artificial muscles (sPAMs) and series pouch motors (SPMs) shorten when pressurized
(B example) tendons or pouch motors located at discrete positions along the body - this is sort of what we do. 
With physical hard stops: Having all the bending concentrated at a single point can limit the usable actuation scenarios, so other tendon actuation designs include a limit on the local bending. In Blumenschein et al. (2018a,b), Gan et al. (2020), and Wang et al. (2020) this was accomplished through physical hard stops placed along the tendon's routed path on the surface of the tube
(C) Preformed - could us if map is known
(D) Passive environment steering - could use partially
(E) Stiffness change - could use

Deploying and reconfiguring structures - e.g. haptics and reconfigurable antennas



- Specific contributions:
-- Characterization of pressurized growing robot load capability
-- New method for adding programmable direction of growth in vine robots
-- Prototype demonstration of grown structures
-- Algorithmic approach demonstrated to plan paths for grown structures through simulations 

